CrescendoNet: A Simple Deep Convolutional Neural Network with Ensemble Behavior

We introduce a new deep convolutional neural network, CrescendoNet, by stacking simple building blocks without residual connections. Each Crescendo block contains independent convolution paths with increased depths. The numbers of convolution layers and parameters are only increased linearly in Crescendo blocks. In experiments, CrescendoNet with only 15 layers outperforms almost all networks without residual connections on benchmark datasets, CIFAR10, CIFAR100, and SVHN. Given sufficient amount of data as in SVHN dataset, CrescendoNet with 15 layers and 4.1M parameters can match the performance of DenseNet-BC with 250 layers and 15.3M parameters. CrescendoNet provides a new way to construct high performance deep convolutional neural networks without residual connections. Moreover, through investigating the behavior and performance of subnetworks in CrescendoNet, we note that the high performance of CrescendoNet may come from its implicit ensemble behavior, which differs from the FractalNet that is also a deep convolutional neural network without residual connections. Furthermore, the independence between paths in CrescendoNet allows us to introduce a new path-wise training procedure, which can reduce the memory needed for training.

==> macros.tex <==
\usepackage{color} % needed for xxx

% Dash command
\newcommand*\dash{\unskip\kern.16667em---\penalty\exhyphenpenalty
        \hskip.16667em\relax
}

\marginparwidth.25in
 % Complex \xxx for making notes of things to do.  Use \xxx{...} for general
 % notes, and \xxx[who]{...} if you want to blame someone in particular.
 % Puts text in brackets and in bold font, and normally adds a marginpar
 % with the text ``xxx'' so that it is easy to find.  On the other hand, if
 % the comment is in a minipage, figure, or caption, the xxx goes in the text,
 % because marginpars are not possible in these situations.
 {\makeatletter
  \gdef\xxxmark{%
    \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
      \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
        \marginpar{\textcolor{red}{xxx}}% not in a caption or minipage, can use marginpar
      \else
        \textcolor{red}{xxx~}% notice trailing space
      \fi
    \else
      \textcolor{red}{xxx~}% notice trailing space
    \fi}
  \gdef\xxx{\@ifnextchar[\xxx@lab\xxx@nolab}
  \long\gdef\xxx@lab[#1]#2{{\bfseries [\xxxmark \textcolor{red}{#2}
  ---{\scshape #1}]}}
  \long\gdef\xxx@nolab#1{{\bfseries [\xxxmark \textcolor{red}{#1}]}}
  % This turns them off:
 \long\gdef\xxx@lab[#1]#2{}\long\gdef\xxx@nolab#1{}%
 }
